Correlating L\'evy processes with Self-Decomposability: Applications to Energy Markets

Based on the concept of self-decomposability, we extend some recent multivariate L\'evy models built using multivariate subordination with the aim of capturing situations in which a sudden event in one market is propagated onto related markets after a certain stochastic time delay. Consequently, we study the properties of such processes, derive closed form expressions for the characteristic function and detail how a Monte Carlo scheme can be easily implemented. We illustrate the applicability of our approach in the context of gas and power Energy markets focusing on the calibration and on the pricing of spread options written on different underlying assets using simulations techniques.

==> Calibration.tex <==
We use a two-steps calibration procedure as in \citet{BB2013} and \citet{SL2010}: firstly, we calibrate the marginal parameters on vanilla products that are usually liquid in many markets. Secondly, since derivatives written on more products are very illiquid, the dependence parameters are estimated fitting the correlation matrix on historical series of the underlying assets.

\subsection{Margins calibration}
Suppose we can observe $n$ vanilla contract prices denoted with $C_{i}$, $i=1,\dots,n$. Denote with $\boldsymbol{\theta}$ the vector of unknown marginal parameters and with  $C_{i}^{\boldsymbol{\theta}}\left(K,T\right)$ model prices. The optimal parameters set $\boldsymbol{\theta}^{*}$ can be found solving:

\begin{equation}
\boldsymbol{\theta}^{*} = \argmin_{\boldsymbol{\theta}} \sum_{i=1}^{n} \left(C_{i}^{\boldsymbol{\theta}}\left(K,T\right) - C_{i}\right)^{2}.
\label{eqn:minimizationproblem_margins}
\end{equation}
Since calibration procedure requires the computation of a large number of derivative prices for different values of $\boldsymbol{\theta}$, we need a very fast option pricing method. To this end, methods based on FFT techniques, as proposed in \citet{CarrMadan99} and \citet{lewis}, are recommended to compute $C_{i}^{\boldsymbol{\theta}}\left(K,T\right)\; i=1,\dots,n$ in each iteration of the minimization algorithm. In our numerical experiment both methods produce very close results, and we choose the method proposed by \citet{CarrMadan99}.

\subsection{Dependence structure calibration}
Once the margins have been fitted, we fit the dependence structure looking at the historical realizations of log-returns of two underlying assets: we denote the market correlation with $\rho_{M}$. Two different approaches can be used: the first one consists of simply observing the correlation of log-returns in the market $\rho_{M}$ and of trying to find $\boldsymbol{\eta}^{*}$ such that:
\begin{equation}
\boldsymbol{\eta}^{*} = \argmin_{\boldsymbol{\eta}} \left(\rho_{\textbf{Y}\left(t,\boldsymbol{\eta}\right)}  - \rho_{M}\right)^{2}.
\label{eqn:minimizationproblem_common}
\end{equation}
where $\boldsymbol{\eta}$ is the set of dependence parameters and $\rho_{\textbf{Y}\left(t,\eta\right)}$ is the correlation of the model: of course, some parameters constraints can be added. 

Another possible approach consists of using the generalized method of moments (\emph{GMM}) as proposed by \citet{Hansen1982}. Since the \chf\ $\phi_{\boldsymbol{Y}\left(t\right)}\left(u_{1},u_{2}\right)$ for the process $\boldsymbol{Y}\left(t\right)$ is available in closed form, it is possible to compute the moment generating function $M\left(u_{1},u_{2}\right)$ and then computing the mixed moments:
\begin{equation}
\mathbb{E}\left[Y_{1}^{n}Y_{2}^{m}\right] = \left. \frac{\partial M^{n+m}\left(u_{1},u_{2}\right)}{\partial u_{1}^{n} \partial u_{2}^{m}}\right|_{\substack{u_{1}=0\\u_{2}=0}}
\label{eqn:GMMequation}
\end{equation}
%_{\substack{u_{1}=0\\u_{2}=0}}
\noindent Then the \emph{GMM} is applied and vector $\boldsymbol{\eta}^{*}$ estimated. 
\par Both methods have advantages and drawbacks. The problem in \eqref{eqn:minimizationproblem_common} is undetermined because we have only one equation and several parameters to fit: for this reason the set of estimated parameters is not unique. In
\eqref{eqn:GMMequation} numerical computation of higher moments lacks of precision if the data-set is not large enough. \\
We have chosen the first presented method because the size of the data-set is not very large and the higher moments computation might be inaccurate.



==> FFTForSpreadOptions.tex <==
%%%%%%%%%%%%%%%%%%%%%
%%%%% CALDANA AND FUSAI %%%%%
%%%%%%%%%%%%%%%%%%%%%

%\section{Fourier method for Spread Options pricing}
The payoff of spread options depends on the difference of two or more underlying assets.
For an in-depth discussion about spread option pricing in log-normal setting one can refer to \citet{Kirk1995} and \citet{Carmona2003}.
\citet{Cheang2008} extended result obtained by \citet{Mar78} to the case of exchange options where both stock price processes contain compound Poisson jump components whereas \citet{Pellegrino2014} applied a three-dimensional Fourier cosine series expansion method in order to price and hedge multiasset spread options. In the more general \Levy\ framework, \citet{hurd2009} proposed a Fourier technique based on the double inversion of the Fourier transform to price spread options.
In contrast, \citet{caldanafusai2016} and \citet{Pellegrino2016} developed an approximated formula based on a single Fourier inversion.
All these techniques require an explicit expression of the \chf\ $\Phi_{T}\left(\boldsymbol{u}\right) = \mathbb{E}\left[e^{i\langle \boldsymbol{u}^{T},\boldsymbol{Y}\left(T\right)\rangle}\right]$  of the joint log-process. 

As shown above, we derived closed form expressions for the \chf’s of all the introduced models. For this reason we can use any of these Fourier methods: we chose anyway the approximated method proposed by \citet{caldanafusai2016} and we refer to their papers for details.

%: here we report only the pricing formula and the \chf\ $\phi_{Y_{1}\left(t\right),Y_{2}\left(t\right)}\left(u_{1},u_{2}\right)$ we used in our paper for the 2D Variance-Gamma process but it can also be used if one has to price derivatives using a Normal Inverse Gaussian multivariate process.\\

% Approximated Formula
%\subsection{An approximated formula for Spread-Options}
Let $S_{1}\left(t\right)$ and $S_{2}\left(t\right)$ be two underlying assets, then the price of an European spread option with maturity $T$ is given by:

\begin{equation}
C_{K}\left(0\right) = e^{-rT} \mathbb{E}\left[\left(S_{1}\left(T\right) - S_{2}\left(T\right) - K\right)^{+}\right]
\nonumber
\end{equation}
%If we define the event $A$:
%
%\begin{equation}
%A = \left\{\omega: \frac{S_{1}\left(T\right)}{S_{2}^{\alpha}\left(T\right)} > \frac{e^{k}}{\mathbb{E}\left(S_{2}^{\alpha}\left(T\right)\right)}\right\}
%\nonumber
%\end{equation}
%the value:
%
%\begin{equation}
%C_{K}^{k,\alpha}\left(0\right) = e^{-rT}\mathbb{E}\left[\left(S_{1}\left(T\right) - S_{2}\left(T\right)-K\right)\mathbbm{1}_{A}\right]
%\nonumber
%\end{equation}
%can be computed in a semi-explicit way and, moreover, $C_{K}^{\alpha,k}\left(0\right)$ is a very good approximation for $C_{K}\left(0\right)$ for suitable choices of $\alpha$ and $k$.\\
Setting $\boldsymbol{u}=\left(u_{1},u_{2}\right)^{T} \in \mathbb{R}^{2}$ and $\boldsymbol{Y}\left(t\right) = \left(\log S_{1}\left(t\right),\log S_{2}\left(t\right)\right)^{T}$ they have the following proposition. 

%\begin{equation*}
%\Phi_{T}\left(\boldsymbol{u}\right) = \Phi_{T}\left(u_{1},u_{2}\right) = \mathbb{E}\left[e^{iu_{1}\log S_{1}\left(T\right) + iu_{2} S_{2}\left(T\right)}\right] = 
%\mathbb{E}\left[e^{i\langle \boldsymbol{u}^{T},\boldsymbol{Y}\left(T\right)\rangle}\right]
%\nonumber
%\end{equation*}

\begin{prop}
\label{prop:caldanafusai}
The approximate spread option value $C_{K}^{k,\alpha}\left(0\right)$ is given in term of a Fourier inversion formula as:

\begin{equation}
C_{K}^{k,\alpha}\left(0\right) = \left(\frac{e^{-\delta k - rT}}{\pi} \int_{0}^{+\infty}e^{-i\gamma k}\Psi_{T}\left(\gamma;\delta,\alpha\right)d\gamma\right)^{+},
\end{equation}
where $\delta$ is the dumping factor and

\begin{equation}
\begin{split}
\Psi_{T}\left(\gamma;\delta,\alpha\right) = \frac{e^{i\left(\gamma-i\delta\right)\log\left(\Phi_{T}\left(0,i\alpha\right)\right)}}{i\left(\gamma - i\delta\right)} \left[\Phi_{T}\left(\left(\gamma -i\delta\right)-i,-\alpha\left(\gamma-i\delta\right)\right) - \right. \\
\left.\Phi_{T}\left(\gamma - i \delta,-\alpha\left(\gamma-i\delta\right)-i\right) - K\Phi_{T}\left(\gamma-i\delta,-\alpha\left(\gamma-i\delta\right)\right)\right]
\end{split}
\nonumber
\end{equation}
and

\begin{equation*}
\alpha  = \frac{F_{2}\left(0,T\right)}{F_{2}\left(0,T\right) + K}, \;
k  = \log\left(F_{2}\left(0,T\right) + K\right),\;
F_{2}\left(0,T\right)  = %\mathbb{E}\left[S_{2}\left(T\right)\right] =
\Phi_{T}\left(0,-i\right)
\end{equation*}

%\begin{align*}
%\alpha & = \frac{F_{2}\left(0,T\right)}{F_{2}\left(0,T\right) + K} \\
%k & = \log\left(F_{2}\left(0,T\right) + K\right)\\
%F_{2}\left(0,T\right) & = \mathbb{E}\left[S_{2}\left(T\right)\right] = \Phi_{T}\left(0,-i\right)
%\end{align*}
\end{prop}
%Observe, moreover, that $F_{2}\left(0,T\right)$ in the previous formulas can be computed in the following way:

%\begin{equation}
%F_{2}\left(0,T\right) = \mathbb{E}\left[S_{2}\left(T\right)\right] = \Phi_{T}\left(0,-i\right)
%\nonumber
%\end{equation}
%A comparison between Monte Carlo method and the proposed Fourier method in Ballotta-Bonfiglioli model with Self-Decomposable subordinators is shown in Figure \ref{fig:MCvsFFT}. We can note that option prices are almost the same and the confirmation is reported in Table \ref{tbl:MCvsFFT}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.3]{./images/MCvsFFTBallottaBonf.eps}
%    \caption{Comparison of Monte Carlo methods for spread options and Fouries method applied to Ballotta and Bonfiglioli model with self-decomposable subordinators.}
%    \label{fig:MCvsFFT}
%\end{figure}


%\begin{table}[ht]
%\centering % SPREAD OPTION PRICING COMPARED MC VS FFT
%\begin{tabular}{ccc}
%\toprule
%$K$ & Monte Carlo & Fourier Method \\ [0.5ex]
%\midrule
%0.0 & 5.96 & 5.97  \\
%0.4 & 5.65 & 5.67  \\
%0.8 & 5.35 & 5.36  \\
%1.2 & 5.06 & 5.07  \\
%1.6 & 4.78 & 4.79  \\
%2.0 & 4.50 & 4.51  \\
%2.4 & 4.24 & 4.25  \\
%2.9 & 3.98 & 3.99  \\
%3.3 & 3.74 & 3.74  \\
%3.7 & 3.50 & 3.51  \\
%4.1 & 3.28 & 3.28  \\
%4.5 & 3.06 & 3.06  \\
%4.9 & 2.86 & 2.85  \\
%5.3 & 2.66 & 2.66  \\
%5.7 & 2.47 & 2.47  \\
%6.1 & 2.30 & 2.29  \\
%6.5 & 2.13 & 2.12  \\
%6.9 & 1.97 & 1.97  \\
%7.3 & 1.82 & 1.82  \\
%7.8 & 1.69 & 1.68  \\
%8.2 & 1.55 & 1.54  \\
%8.6 & 1.43 & 1.42  \\
%9.0 & 1.32 & 1.31  \\
%9.4 & 1.21 & 1.20  \\
%9.8 & 1.11 & 1.10  \\
%10.2 & 1.02 & 1.01  \\
%10.6 & 0.94 & 0.92  \\
%11.0 & 0.86 & 0.84  \\
%11.4 & 0.79 & 0.77  \\
%11.8 & 0.72 & 0.70  \\
%12.2 & 0.66 & 0.64  \\
%12.7 & 0.60 & 0.58  \\
%13.1 & 0.55 & 0.53  \\
%13.5 & 0.50 & 0.48  \\
%13.9 & 0.45 & 0.44  \\
%14.3 & 0.41 & 0.40  \\
%14.7 & 0.38 & 0.36  \\
%15.1 & 0.34 & 0.33  \\
%15.5 & 0.31 & 0.30  \\
%%15.9 & 0.28 & 0.27  \\
%%16.3 & 0.26 & 0.24  \\
%%16.7 & 0.23 & 0.22  \\
%%17.1 & 0.21 & 0.20  \\
%%17.6 & 0.19 & 0.18  \\
%%18.0 & 0.17 & 0.16  \\
%%18.4 & 0.16 & 0.15  \\
%%18.8 & 0.14 & 0.13  \\
%%19.2 & 0.13 & 0.12  \\
%%19.6 & 0.12 & 0.11  \\
%%20.0 & 0.11 & 0.10  \\
%\bottomrule
%\end{tabular}
%\caption{Comparison of Monte Carlo and Fourier technique applied to compute the price of spread options in Ballotta-Bonfiglioli's model with self-decomposable subordinators.} % title of Table
%\label{tbl:MCvsFFT} % is used to refer this table in the text
%\end{table}

%\textcolor{red}{Quando vai a fare questa figura NON bloccare il parametro $a$ nella fase di calibrazione ma abbassa, piuttosto, la correlazione dei processi. Attendo perchè, affinchè vada tutto bene, è NECESSARIO che le condizioni di convoluzione siano soddisfatte in maniera puttosto stingente ovvero $\sim 0.004$.}\\
%Refert to \citet{caldanafusai2016} and  \citet{Pellegrino2016} for an extensive analysis of the topic. 

==> FinancialModel.tex <==
\label{sec:finmodel}
Similar to \citet{CT2003}, we consider financial markets driven by exponential \Levy\ processes $\boldsymbol{Y}\left(t\right)$ defined in the previous sections. The price of the asset $S_j(t)$ at time $t$ can be defined as follow:
\begin{equation}
S_{j}\left(t\right) = S_{j}\left(0\right) e^{rt + \omega_{j} t + Y_{j}\left(t\right) }
\label{eqn:themodel}
\end{equation}
where $r$ is the risk-free rate and $\omega_{j}$ is the drift corrector. By introducing a new source of randomness, the market is incomplete and we do not have a unique equivalent martingale measure (\citet[Chapter 5]{Shreve04}). Non-arbitrage conditions can be obtained setting:
\begin{equation}
\omega_{j} = -\varphi\left(-i\right)
\label{eqn:omegaexpr}
\end{equation}
If we focus on the Variance Gamma process with parameters $\left(\mu_{j},\sigma_{j},\nu_{j}\right)$ we obtain:
\begin{equation}
\omega_{j} = \frac{1}{\nu_{j}} \log \left(1 - \frac{\sigma_{j}^2 \nu_{j}}{2} - \mu_{j} \nu_{j}\right).
\nonumber
\end{equation}
Once that the complete theoretical framework has been derived, in next session we apply our model to real markets and check its performance.

==> SimulationAlgo.tex <==
In this section we present algorithms to simulate the stochastic processes introduced in previous sections. The choice of Gamma process was driven by the fact that we know how to efficiency simulate the \arem\ $Z_{a}\left(t\right)$. We could also adopt an Inverse Gaussian law, that is \sd\ as shown in \citet{Halgreen1979}: however, an efficient way to simulate its \arem\  is not available at the moment. A numerical MC scheme to simulate a Variance Gamma process with parameters $\left(\mu,\sigma,\nu \right)$ is easy to implement and can be found in \citet[Algorithm~ 6.11]{CT2003}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% VARIANCE GAMMA SIMULATION %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Variance-Gamma Simulation}
%The numerical method to simulate a Gamma process with parameters $\left(\mu,\sigma,\nu \right)$ is can be easly implemented and can be found in \citet[Algorithm~ 6.11]{CT2003}.
%The algorithm is reported in Box \ref{algo:VGSimulation} can be used to simulate a %Variance-Gamma process and it is proposed by \citet{CT2003}.


%\begin{algorithm}
%\caption{Simulating a Variance Gamma on a equispaced time grid}\label{algo:VGSimulation}
%Simulation of $\left(Y\left(t_{1}\right),\cdots,Y\left(t_{n}\right)\right)$ in quispaced time grid with step $\Delta t$, $t_{1},\cdots,t_{n}$: a discretized of the Variance-Gamma process with parameters $\left(\mu, \sigma,\nu\right)$
%
%\begin{algorithmic}[1]
%\State Simulate $n$ independent gamma \rv's $\Delta S_{1},\cdots,\Delta S_{n}$ with parameters $\left(\frac{\Delta t}{\nu},\frac{1}{\nu}\right)$.
%\State Simulate $n$ i.i.d. $\mathcal{N}\left(0,1\right)$ \rv's $N_{1},\cdots,N_{n}$. Set $\Delta Y_{i} = \sigma N_{i}\sqrt{\Delta S_{i}} + \mu \Delta S_{i}$ for all $i$.
%\State The discretized trajectory is $Y\left(t_{i}\right) = \sum_{k=1}^{i}\Delta X_{i}$
%\end{algorithmic}
%\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% a-REMINDER %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{$Z_{a}\left(t\right)$ Simulation}
In order to simulate \sd\ dependent Gamma processes $H_{1}\left(t\right)$ and $H_{2}\left(t\right)$ defined in \eqref{eqn:subordinatorsSD}, one must know how to simulate a r.v. $Z_{a}\left(t\right)$. \citet{cs20} and \cite{cs20_2} have shown that the \arem\ of a Gamma distribution $\Gamma\left(\alpha,\lambda\right)$ can be simulated taking:
\begin{equation*}
Z_{a} = \sum_{j=1}^{S} X_{j}
\end{equation*}
where

\begin{equation*}
S \sim \mathfrak{B}\left(\alpha,1-a\right) \quad X_{j} \sim \mathfrak{E}\left(\lambda/a\right) \quad X_{0} = 0 \quad \boldsymbol{P}-a.s.
\end{equation*}
$\mathfrak{B}\left(\alpha,1-a\right)$ denote a Polya or negative binomial distribution and $\mathfrak{E}\left(\lambda/a\right)$ denotes an exponential distribution. Algorithm \ref{alg:sd} shows how to simulate $Z_{a}\left(t\right)$ over a fixed time grid $t_0, t_1,\dots, t_N$, $\Delta t_n = t_n - t_{n-1}\,,\; n=1,\dots,N $.
\begin{algorithm}
	\caption{ }\label{alg:sd}
	\begin{algorithmic}[1]
		\For{ $n=1, \dots, N$}
		\State $b\gets B\sim \mathfrak{B}(\alpha,1-a)$ \Comment{Generate a Polya $(\alpha,1-a)$ \rv}
		\State $\Delta Z_{n}^{a} \gets Z_a^{(n)}\sim \mathfrak{E}_{b}\left(\,\!^\lambda/_a\right)$; \Comment{ Generate an Erlang \rv\ with rate $\lambda/_a$}
		\State $Z\left(t_{n}\right) = Z\left(t_{n-1}\right) + \Delta Z_{n}^{a}$.
		\EndFor
	\end{algorithmic}
\end{algorithm}

\noindent Different types of dependent  \sd\ subordinators varying $a$ are shown in Figure \ref{fig:sdsubordinators}.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{./images/SD_subordinators.eps}
    \caption{Correlated subordinators $H_{1}\left(t\right)$ and $H_{2}\left(t\right)$ with different values of $a$.}%The increment of $H_{1}\left(t\right) \sim \Gamma\left(\Delta t \cdot A,B\right)$ with $A=7.2$, $B=1$ and $\Delta t = 1/365$.}
    \label{fig:sdsubordinators}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% SEMERARO MODEL SIMULATION %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Semeraro's Process Simulation Algorithm}
%\subsection{2D- VG Processes Simulation Algorithms}
Algorithms \ref{algo:SemeraroSimulation}, \ref{algo:SLAlgorithm}, \ref{algo:BBAlgorithm} show how to simulate processes defined, respectively, in Section \ref{sec:SSD}, Section \ref{sec:LSSD} and Section \ref{sec:BBSD}.
%Algorithm \ref{algo:SemeraroSimulation} shows how to simulate a bivariate process as the one proposed by \citet{Semeraro2008} extended with \sd\ subordinators.

\begin{algorithm}
\caption{\sd-Semeraro model}\label{algo:SemeraroSimulation}
Simulation of a bivariate Variance Gamma $\left(Y_{1}\left(t\right),Y_{2}\left(t\right)\right)$ in equally-spaced time grid with step $\Delta t$, $t_{1},\cdots,t_{i},\cdots,t_{n}$.
\begin{algorithmic}[1]
\State Simulate $n$ \iid\ gamma \rv's $\Delta I_{j,i} \sim \Gamma \left(\Delta t\left(\frac{1}{\alpha_{j}}-A\right),\frac{1}{\alpha_{j}}\right)$, $j=1,2$, $i=1,\dots,n$.
\State Simulate $n$ \iid\ gamma \rv's $\Delta H_{1,i} \sim \Gamma \left(\Delta t\cdot  A,1\right)$, $i=1,\dots,n$. 
\State Simulate $n$ \iid\ $\Delta Z_{a,i}$, $i=1,\dots,n$ \rv's as \arem\ of a Gamma distribution $\Gamma \left(\Delta t\cdot A,1\right)$ using Algorithm \ref{alg:sd}.
\State Set $\Delta H_{2,i} = a \Delta H_{1,i} + \Delta Z_{a,i}$, $i=1,\dots,n$.
\State Set $\Delta G_{j,i} = \Delta I_{j,i} + \alpha_{j} \Delta H_{j,i}$, $j=1,2$, $i=1,\dots,n$.
\State Simulate $n$ \iid\ standard normal \rv's,  $N_{i}\; i=1,\dots,n$
\Statex Set $\Delta Y_{j,i} = \sigma_{j} N_{i}\sqrt{\Delta G_{j,i}} + \mu_{j} \Delta G_{j,i}$, $j=1,2$, $i=1,\dots,n$.
\State The discretized trajectories are $Y_{j}\left(t_{i}\right) = \sum_{k=1}^{i}\Delta Y_{j,k}$, $j=1,2$.
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% SEMERARO - LUCIANO MODEL SIMULATION %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\subsection{Semeraro-Luciano's Process Simulation Algorithm}
%Algorithm \ref{algo:SLAlgorithm} shows how to simulate a bivariate process as the one proposed by \citet{SL2010} extended with \sd\ subordinators.

\begin{algorithm}
\caption{\sd-Semeraro-Luciano  model}\label{algo:SLAlgorithm}
Simulation of a bivariate Variance Gamma $\left(Y_{1}\left(t\right),Y_{2}\left(t\right)\right)$ in equally-spaced time grid with step $\Delta t$, $t_{1},\cdots,t_{i},\cdots,t_{n}$.
\begin{algorithmic}[1]
\State Simulate $n$ \iid\ Gamma \rv's $\Delta I_{j,i} \sim \Gamma \left(\Delta t\left(\frac{1}{\alpha_{j}}-A\right),\frac{1}{\alpha_{j}}\right)$, $j=1,2$, $i=1,\dots,n$.
\State Simulate $n$ independent gamma \rv's $\Delta H_{1,i} \sim \Gamma \left(\Delta t\cdot  A,1\right)$, $i=1,\dots,n$.
\State Simulate $n$ independent $\Delta Z_{a,i}$, $i=1,\dots,n$ \rv's as \arem\ of a Gamma distribution $\Gamma \left(\Delta t\cdot A,1\right)$ using Algorithm \ref{alg:sd}.
\State Set $\Delta H_{2,i} = a \Delta H_{1,i} + \Delta Z_{a,i}$, $i=1,\dots,n$
\State Simulate $n$ \iid\ standard normal \rv's $N_{j,i}$, $j=1,2$, $i=1,\dots,n$
\State Set $\Delta Y_{I_{j,i}} = \sigma_{1} N_{j,i}\sqrt{\Delta I_{j,i}} +\mu_{j} \Delta I_{j,i}$.
\State Simulate $n$ jointly standard normal \rv\ $\left(\Delta W_{1,1}^{\rho},\Delta W_{2,1}^{\rho}\right)$,$i=1,\dots,n$ with correlation $\sqrt{a}$.
\State Simulate $n$ standard normal \iid\ \rv's $W_{3,1},\cdots,W_{3,n}$, $i=1,\dots,n$.
\State Set: $\Delta Y_{H_{1},i} = \sqrt{\alpha_{1}}\sigma_{1}\Delta W_{1,i}^{\rho} \sqrt{\Delta H_{1,i}} + \alpha_{1}\mu_{1}\Delta H_{1,i}$, $i=1,\dots,n$.
\State Set: $\Delta Y_{H_{2},i} = \sqrt{\alpha_{2}}\sigma_{2}\left(\Delta W_{2,i}^{\rho} \sqrt{a \Delta H_{1,i}}+ \sqrt{\Delta Z_{a,i}} \Delta W_{3,i}\right) + \alpha_{2}\mu_{2}\Delta H_{2,i}$, $i=1,\dots,n$.
\State Set $Y_{H_{j}}\left(t_{i}\right)  =\sum_{k=1}^{i} \Delta Y_{H_{j},k} $, $j=1,2$, $i=1,\dots,n$.
\State Set $Y_{I_{j}}\left(t_{i}\right)  =\sum_{k=1}^{i} \Delta Y_{I_{j},k} $, $j=1,2$, $i=1,\dots,n$.
\State Set $Y_{j}\left(t_{i}\right) = Y_{I_{j}}\left(t_{i}\right) + Y_{H_{j}}\left(t_{i}\right) $, $j=1,2$, $i=1,\dots,n$.
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% BALLOTTA-BONFIGLIOLI MODEL SIMULATION %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\subsection{Ballotta-Bonfiglioli's Process Simulation Algorithm}
%Algorithm \ref{algo:BBAlgorithm} shows how to simulate a bivariate process as the one proposed %by \citet{BB2013} extended with \sd\ subordinators.

\begin{algorithm}
\caption{\sd-Ballotta-Bonfiglioli model}\label{algo:BBAlgorithm}
Simulation of a bivariate Variance Gamma $\left(Y_{1}\left(t\right),Y_{2}\left(t\right)\right)$ in equally-spaced time grid with step $\Delta t$, $t_{1},\cdots,t_{i},\cdots,t_{n}$.
\begin{algorithmic}[1]
\State Simulate a Variance Gamma process $X_{j}\left(t_{i}\right)$ with parameters $\left(\beta_{j},\gamma_{j},\nu_{j}\right)\; j=1,2$. %using algorithm in Box \ref{algo:VGSimulation}.
\State Simulate $n$ \iid\ Gamma \rv's $\Delta H_{1,i} \sim \Gamma \left(\frac{\Delta t}{\nu_{R}} ,\frac{1}{\nu_{R}}\right)$, $i=1,\dots,n$.
\State Simulate $n$ \iid\ \rv's $\Delta Z_{a,i}$ as \arem\ of a Gamma distribution $\Gamma \left(\frac{\Delta t}{\nu_{R}} ,\frac{1}{\nu_{R}}\right)$, $i=1,\dots,n$.
\State Set $\Delta H_{2,i} = a \Delta H_{1,i} + \Delta Z_{a,i}$, $i=1,\cdots,n$.
\State Simulate $n$ standard normal \iid\ \rv's $N_{j,i}$, $j=1,2$, $i=1,\cdots,n$.
\State Set $\Delta R_{1,i} = \gamma_{R_{1}} N_{1,i}\sqrt{\Delta S_{1,i}} +\beta_{R_{1}} \Delta S_{1,i}$, $i=1,\dots,n$.
\State Simulate $n$ \iid\ standard normal \rv's $N_{3,1},\cdots,N_{3,n}$ correlated with $N_{1,i}\; i=1,\cdots,n$ with correlation $\sqrt{a}$.
\State Set $\Delta R_{2,i} = \gamma_{R_{2}}\left(N_{3,i}\sqrt{a\Delta S_{1,i}}+\sqrt{\Delta Z_{a,i}}N_{2,i}\right) +\beta_{R_{2}} \Delta S_{2,i}$, $i=1,\cdots,n$.
\State Set $R_{j}\left(t_{i}\right) = \sum_{k=1}^{i} \Delta R_{j,k}$, $j=1,2$, $i=1,\dots,n$.
\State Set $Y_{j}\left(t_{i}\right) = X_{j}\left(t_{i}\right) + R_{j}\left(t_{i}\right)$, $j=1,2$, $i=1,\dots,n$.
\end{algorithmic}
\end{algorithm}

